Optimal Behavior Prior: Data-Efficient Human Models for Improved Human-AI Collaboration

AI agents designed to collaborate with people benefit from models that enable them to anticipate human behavior. However, realistic models tend to require vast amounts of human data, which is often hard to collect. A good prior or initialization could make for more data-efficient training, but what makes for a good prior on human behavior? Our work leverages a very simple assumption: people generally act closer to optimal than to random chance. We show that using optimal behavior as a prior for human models makes these models vastly more data-efficient and able to generalize to new environments. Our intuition is that such a prior enables the training to focus one's precious real-world data on capturing the subtle nuances of human suboptimality, instead of on the basics of how to do the task in the first place. We also show that using these improved human models often leads to better human-AI collaboration performance compared to using models based on real human data alone.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/10-intro.tex <==
\section{Introduction}

% \MicahComment{tasks vs models vs inferences}
% \MicahComment{masking schemes / input maskings}

% \orrp{Figure out \masking vs. masking vs. masking schemes etc.}

\label{sec:intro}
Masked language modeling~\citep{devlin2018bert} is a key technique in natural language processing (NLP). Under this paradigm, models are trained to predict randomly-masked subsets of tokens in a sequence. For example, during training, a BERT model might be asked to predict the missing words in the sentence ``yesterday I \longblank{} cooking a \longblank''. Importantly, while unidirectional models like GPT~\citep{radford2018improving} are trained to predict the next token conditioned only on the left context, bidirectional models trained on this objective learn to model both the left \emph{and} right context to represent each word token. This leads to richer representations that can then be fine-tuned to excel on a variety of downstream tasks~\citep{devlin2018bert}.

Our work investigates how masked modeling can be a powerful idea in sequential decision problems. Consider a sequence of states $s$ and actions $a$ collected across $T$ timesteps $s_1,a_1,\dots,s_T,a_T$. If we consider each state and action as tokens of a sequence (analogous to words in NLP) and mask the last action $(s_1,a_1,s_2,a_2,s_3,\shortblank)$, then predicting the missing token $a_3$ amounts to a Behavior Cloning prediction with two timesteps of history \citep{pomerleau_efficient_1991}, given that this masking corresponds to the inference $\Prob{a_3 | s_{1:3}, a_{1:2}}$. From this perspective, training a model to predict missing tokens from all \maskings of the form $(s_1,a_1,\dots,s_{t}, \shortblank, \dots, \shortblank)$ 
for all $t \in [1, \dots, T]$ 
corresponds to training a Behavior Cloning (BC) model.

In this work, we introduce the \fb{} framework: \textbf{Uni}fied Inferences in Sequential Decision Problems via 
% \textbf{Bi}directional \textbf{T}ransformers \MicahComment{fix this!}
\textbf{\texttt{[MASK]}}\!ings, where inference tasks are expressed as \emph{\masking schemes}. Through this framework, commonly-studied tasks such as goal or waypoint conditioned BC~\citep{ding_goal-conditioned_2020, rhinehart_precog_2019}, offline reinforcement learning (RL) \citep{levine2020offline}, forward or inverse dynamics prediction \citep{ha_world_2018, christiano_transfer_2016, chen_transdreamer_2022}, initial-state inference \citep{shah_preferences_2019}, and others are unified under a simple sequence modeling paradigm.
In contrast to standard approaches that train a model for each inference task, we show how this framework naturally lends itself to multi-task training: a single \fb{} model can be trained to perform a variety of tasks out-of-the-box by appropriately selecting sequence maskings at training time.

We test this framework in a gridworld navigation task and a continuous control environment. First, we train a \fb model by sampling from the space of all possible maskings at training time (random masking) and show how this scheme enables a single \fb{} model to perform BC, reward-conditioning, waypoint-conditioning, and more by conditioning on the appropriate subsets of states, actions, and rewards. We then systematically analyze how the masking schemes seen at training time affect downstream task performance. Training on random masking generally does not compromise single-task performance, and in fact can outperform models that only train on the task of interest. In the continuous control environment, we confirm that a model trained with random masking and fine-tuned on BC or RL outperforms models specialized to those tasks.
%However, this is not always the case -- in experiments in a continuous control environment, we find that training on random maskings does incur in a performance hit. However, by fine-tuning these random-masking pre-trained models, one can recover the lost performance and surpass single-task models.

Our results suggest that expressing tasks as sequence maskings with the \fb{} framework may be a promising unifying approach to building general-purpose models capable of performing many inference tasks in an environment \cite{foundation}, or simply offer an avenue for building better-performing single-task models via unified multi-task training.

In summary, our contributions are:

\begin{enumerate}
    \item We propose a new framework, \fb{}, that unifies inference tasks in sequential decision problems as different masking schemes in a sequence modeling paradigm.
    \item We demonstrate how randomly sampling masking schemes at training time produces a single multi-inference-task model that can do BC, reward-conditioning, dynamics modeling, and more out-of-the-box.
    \item We test how training on many tasks affects single-task performance and show how fine-tuning models trained with random masking consistently outperforms single-task models.
    \item We show how the insights we have gained while developing our choice of \fb architecture can be used to improve other state-of-the-art methods.
\end{enumerate}

% We next investigate how a \fb{} can excel even when evaluated on a single task of interest, where masked prediction can serve as a form of data augmentation at training time, where predicting randomly masked tokens amounts to supervising the model with many different tasks beyond next-token prediction. \JessyComment{kind of speculative unless we can back this up somehow?}\MicahComment{i think that the rnd masking schemes working better on Maze/Mujoco than non-random ones kind of show that} On \todo{Mujoco, Atari, and the Bleeding Edge game environment}, we show that pre-training a bidirectional model with the masked objective \todo{outperforms the Decision Transformer} in the low-data regime, while \todo{matching its performance} in the high-data regime. \MicahComment{add more info about Maze and update other envs}

% In summary, in this work we propose \fb, a framework for flexibly defining and training models which: \textbf{1)} are naturally able to represent any inference task and support multi-task training in sequential decision problems, \textbf{2)} match or surpasses the performance of single-task models after multi-task\orrpfn{Drop ``multi-task'' for flow? It was stated above.} pre-training, and almost always surpasses them after fine-tuning.

% Our results align with the finding in other domains that the paradigm of pre-training on a self-supervised objective and then fine-tuning for a specific task is a strong approach to building general-purpose models, though it might be surprising that random masking performs well (cf. \citealt{levine2020pmi}).\orrpfn{\cite{levine2020pmi} also use random masking. It's just that their maskings are randomly sampled from a clever distribution, whereas ours is almost uniform. If we could say ``uniformly random'' here that would be simple, but that's not entirely true. It's also not about entropy. It's about how it's not principled, I guess. Leaving it as ``random'' for now (if you know you get it, if you don't know it doesn't matter).} That said, our main conceptual contribution is a unified framework that encompasses many common tasks in sequential decision problems, which we show is elegantly and practically applicable.


% random somewhat surprising that works at all even in simple environment, but generally not surprising that this all works. what's exciting to recognizing this way of thinking about things and thinking of applying it

% While our analysis (especially for the more complex environments) is preliminary, we believe our approach provides exciting and promising results which warrant further investigation and are worth sharing with the rest of the research community.

==> sections/11-intro-old-notes.tex <==
% \MicahComment{Options for the introduction: 1) bringing bidirectionality and random masking from NLP to sequential decision processes; 2) proposing foundation models for sequential decision problems; 3) building on top of DT-type work; 4) multi-task literature, training on so many tasks that you learn to generalize to unseen ones}

% \MicahComment{One possible way to merge all three is: A perspective that has gaining traction is that of foundation models. In particular, in NLP has seen success with BERT. We build on top of single-task models for sequential decision problems such as DT, incorporating some of the insights of NLP to propose \fb{}.}

% \MicahComment{I don't really like foundation models \url{https://twitter.com/mer__edith/status/1429832405091856397}, but in a way there's no way to escape that}

%Recently there has been work on modeling sequential decision problems with transformers \citep{chen_decision_2021, janner_reinforcement_2021}. They use a decoder architecture (GPT) because of the forward-in-time character of most of their tasks but we can also use bi-directional models such as BERT, when used with appropriate masking. We show how that unlocks various additional modalities of inference that might be of interest, and enables to train a single model which is able to perform many different inference tasks, 
% Goal-conditioned behavior generation is enabled.
% Generation because it can be used both to do "RL" and IL.


Recent Success of DT - No need to constrain sequential decision models in the same way as NLP. What are the opportunities in sequential decision modelling when considering bidirectional models?

why limit ourselves to uni-directional? by using bi-directional, 1) train time, 2) test-time, and also enables us to explore potential for large models like in NLP


Masked Language Modeling \citep{devlin2018bert}, can apply to RL and sequential decision-making problems more broadly. Modeling bidirectional context has proven to be an important component of rich representations in NLP, where intuitively both the left and right context are useful for building the representation of a text token. In this work, we apply bidirectional transformers and masking schemes to sequential decision problems, leading to the surprising conclusion that in this context, masking is arguably more powerful than in language: while in language, masking was just an expedient for obtaining good representations (the applications we are interested in are not ``filling in the blanks'' with BERT), in sequential decision problems every masking scheme can have value in its own right as a meaningful task.

==> sections/20-related-work.tex <==
\section{Related Work}

%The successes of modern natural language processing (NLP) techniques have motivated efforts to apply similar ingredients -- unsupervised pre-training and Transformers~\cite{vaswani2017attention} -- to reinforcement learning (RL). Recent work has shown that GPT-style~\cite{radford2018improving} Transformer models can achieve state-of-the-art performance on offline RL benchmarks~\citep{chen_decision_2021, janner_reinforcement_2021}. A natural question is to ask to what extent the other lessons of unsupervised pre-training can be brought to bear on sequential decision-making problems.
% \JessyComment{maybe work on pretraining-finetuning paradigm}
% \MicahComment{one big issue of the related work currently is that it hyperfocuses on RL rather than the other tasks, when we don't even mention RL in the intro and barely throughout the paper}

\prg{Transformer models.} The great successes of transformer models~\citep{vaswani2017attention} in other domains such as NLP~\citep{devlin2018bert,radford2018improving,brown2020language} and computer vision~\citep{dosovitskiy2020vit,he2021masked} motivates our work. Using transformers in RL and sequential decision problems has proven difficult due to the instability of training~\citep{parisotto2020stabilizing}, but recent work has investigated using transformers in model-based RL~\citep{chen_transdreamer_2022}, motion forecasting~\citep{ngiam_scene_2021}, learning from demonstrations~\citep{recchia2021teaching}, and tele-operation~\citep{clever2021assistive}. %\citep{ngiam_scene_2021} in particular already recognized the flexibility afforded by BERT-like architectures that enable a single model architecture to be trained for multiple tasks. While they also perform multi-task training, they restrict themselves to single tasks of interest rather than training for ``all tasks'' through randomized masking. Another important difference is that their architecture is single-task for motion prediction in the autonomous driving setting, and as such only consider ``state'' predictions, rather than full sequential decision problems.
% We instead focus on forming a unifying framework for tasks in sequential decision problems.
\sm{note downsides of these work / opportunities that our work enables: what does ours do that others does not? most obvious one is that they are often deployed as 1 model : 1 task, whereas we do 1 model : many tasks}

\prg{The utility of randomized masking.} In addition to being used as one of the main training objectives for BERT (the ``cloze task'', \cite{devlin2018bert}), the flexibility afforded by randomized masking in bidirectional models has been utilized in other previous works applied to language \citep{ghazvininejad2019maskpredict,mansimov2019generalized} and vision \citep{chang2022maskgit} -- mostly for the purpose of speeding up auto-regressive decoding, which is not our focus. Concurrent work has also explored using random masking for model-flexibility for probabilistic programming languages \cite{Wu2022FoundationPF}. In the context of language generation \cite{Tay2022UnifyingLL} provides a framework for thinking about different masking schemes.

\prg{Sequential decision-making as sequence modeling.} Previous and concurrent work \citep{chen_decision_2021,janner_reinforcement_2021, Lee2022MultiGameDT} shows how to use GPT-style (causally-masked) transformers to directly generate high-reward trajectories in an offline RL setting.
%Subsequent work has investigated how to apply this formulation to offline multi-agent problems~\cite{meng2021offline}.
We expand our focus to many tasks that a sequence modeling perspective enables, including but not restricted to offline RL. 
%Unlike this line of work, we focus on many tasks that a sequence modeling perspective enables one to do, rather than just offline-RL. 
Although previous work has cast doubt on the necessity of using transformers to achieve good results in offline RL~\citep{emmons_rvs_2021}, we note that offline RL~\cite{levine2020offline} is just one of the various tasks we consider.
Concurrent work to ours generalizes the left-to-right masking in the transformer to condition on future trajectory information for tasks like state marginal matching~\citep{furuta2021generalized} and multi-agent motion forecasting~\citep{ngiam_scene_2021}. In contrast, we systematically investigate how a single bidirectional transformer can be trained to perform arbitrary downstream tasks in more complex settings than motion forecasting---i.e., we also consider agent actions and rewards in addition to states. 
The main thing that sets us apart from these works is a systematic view of all tasks that can be represented by this sequence-modeling perspective, and a detailed investigation of how different multi-task training regimes compare.
% \sm{should we just combine this paragraph with the transformer models section? that one seems really short and closely ties into this paragraph}\MicahComment{I feel like that one is just kind of introducing the breadth of work using transformers, while here we focus on the couple of works which are most related to ours}
%\sm{fair! i realize now that related work is kind of both background and related work. in that case, agree that the current decomposition is fine.}

\prg{Self-supervised learning for sequential decision problems.}
Training on random maskings of one's data can be considered as a form of self-supervised learning. Previous work on self-supervised learning mostly focuses on improving RL by  training models on auxiliary objectives, such as state dynamics prediction~\citep{sekar2020planning} or intrinsic motivation~\citep{pathak2017curiosity}. % can lead to improved downstream performance.
% We note that the notion of ``task'' in the multi-task literature for RL~\citep{notorrp} typically refers to an MDP with an associated reward structure (e.g., picking up a cup vs. pouring water). However, we use ``task'' to refer more generally to an \emph{inference} or \emph{prediction task}, where RL (the task of generating trajectories that achieve high reward) is just one instantiation of the many tasks we consider (behavior cloning, backwards inference, etc.). 
Typically, to accomplish the tasks we consider, prior work relies on single-task models: for example, goal-conditioned imitation learning \citep{ding_goal-conditioned_2020}, RL~\citep{kaelbling1993learning}, waypoint-conditioning \citep{rhinehart_precog_2019}, property-conditioning~\citep{zhan2020learning, furuta2021generalized}, or dynamics model learning~\citep{ha_world_2018, christiano_transfer_2016}.
% \MicahComment{https://www.nature.com/articles/s41586-019-1724-z I forgot why i added this here -- maybe had to do with property-conditioning}
Concurrent works~\citep{gato, Lee2022MultiGameDT} scale up transformers to handle inputs from a large variety of environments (which they call games or ``tasks'' -- \textit{which is different from our usage of the word!}).
We instead demonstrate how sequence modeling can be a unifying framework for formulating and performing any inference task within an environment with a single model.

% \sm{also, may be worth making this task distinction earlier, rather than in the related work section.}\MicahComment{earlier there doesn't really seem to be a clear place where it fits in. Thought it would make sense to talk about when we talk about other multi-task work and our relationship to that}
% bidirectional trajectory prediction~\cite{yao2021bitrap}

% \item transfer learning w/ dt~\cite{boustati2021transfer} Also unpublished but probably should add

% \item lfd w/ transformers~\cite{recchia2021teaching}

% Note that \textit{each possible input masking scheme for a sequence corresponds to a specific inference task} that we are asking the network to be able to perform.

% Recent works that applied transformers to sequential decision problems \cite{} do so without \mask{} tokens, but by instead using GPT-style causal-masking in the self-attention.\MicahComment{make difference between these names clear} Their objective has been to train single-task models to perform a single task -- offline RL.
% We follow their suit in also considering states, actions, and rewards as input tokens to the model. 
% However, by using bidirectional transformers, we are able to use \mask{} tokens in order to train the same model to be able to perform multiple tasks.

% \prg{BERT for sequence generation} In NLP, BERT is not usually used for language generation, although it has been attempted~\citep{wang2019bert}, as it's generally considered to perform worse than GPT-based models for this task. Even though we expect this to be the case also in sequential decision problems, we find that the benefit of the data-augmentation and better representations enabled by using a bidirectional model outweighs the cost.\MicahComment{update this later}
% \sm{this seems maybe more like background? also, do we even need to discuss this as a subsection or can we potentially just briefly mention this somewhere (if it's necessary to include at all?)?}

% \prg{Auxiliary tasks for improved predictions} The idea of requesting one's model to perform extra tasks to the one we are interested in, in order to improve representations, is not new. We find this in RL \cite{jaderberg2016reinforcement, akkaya2019solving,laskin2020curl}; in vision \citet{he2021masked} also applies masking schemes to vision problems, but similarly to NLP this is just for the purpose of increased accuracy on a single downstream task, which can be traced back to the image inpainting line of work in vision \cite{elharrouss2020image}. And in multi-purpose approaches such as \cite{oord2018representation}.

% \prg{Transformers for multi-agent motion forecasting.} Various works have considered the problem of multi-agent motion forecasting in the Autonomous Vehicle domain: most literature deals with single-agent motion prediction (assuming each agent is independent) \citep{saa}, but recent papers that have focused on joint motion prediction \citep{rhinehart_precog_2019, ngiam_scene_2021}. The most related work among these is \citep{ngiam_scene_2021}, who use a custom transformer architecture for the AV setting and focus on the problem of conditional multi-agent motion forecasting. Our work can be thought of as generalizing their approach to a 1) setting with actions, 2) higher dimensional state predictions than just $x,y$ positions and heading, 3) propose an architecture that is not AV-specific, and 4) we showcase additional conditional generation schemes. Multiagent imputation \citep{deepmind_soccer}

% \citep{shang2021starformer} Not yet published

% Maybe add schmidthuber work on RvS and full section on RvS -- if this is what we focus on in mujoco etc.



==> sections/30-model.tex <==
% ERT~\citep{devlin2018bert} is bidirectional in that every output token depends on every input token, rather than only the tokens preceding it in the input (as caused by the causal-masking in the self-attention). To further stress this point, BERT models have no masking in the self-attention. One objective used during BERT's training is the ``cloze task'', which involves randomly replacing some input tokens (e.g. words) with a \mask{} token, which are then predicted in the output. Essentially, the network is trained to ``fill in the blanks'' whenever a \mask{} token is encountered. \textbf{N.B.} the \mask{} tokens we are referring to here are \textit{input masks} (a direct modification of the input at pre-inference time) which have nothing to do with the \textit{self-attention masks} mentioned before (which dictate which outputs can see which inputs). 
% % In BERT's cloze training task, for each input token which is masked with a \mask{} token, the transformer outputs a prediction based on all other inputted context: essentially, the network is trained to ``fill in the blanks''. %One thing to note is that this \mask{} token approach is only possible due to the bidirectional nature of self-attention in BERT -- masking the first token would not make sense in a model with self-attention with causal-masking.\MicahComment{better explain}
% In the context of BERT, \MicahComment{one isn't interested in this task specifically!!}this has been found to be an effective self-supervised learning objective which improves the quality of BERT's word representations. In this work, we apply BERT's cloze task philosophy to sequential decision problems and use such training not to obtain better representations -- but a \textit{single} model which is able to perform many inference types.

% \prg{Notation.} \MicahComment{notation: masking scheme (function), masking (token-level/sequence-level instance). Not sure if we want to clarify this somewhere. Not sure if we can improve this also}
% \sm{is it easier to just have a table that we refer to for this if we think the notation will be confusing?}


\section{The \fb{} Framework}
We introduce the \fb framework. In \Cref{sec:masking_schemes} we propose a unifying interpretation of inference tasks in sequential decision problems as masking schemes. In \Cref{sec:training} we describing different ways of training \fb{} models, an provide hypotheses about their efficacy.

We consider trajectories as sequences of states, actions, and (optionally) property tokens: $\tau = \{ (s_0, a_0, p_0), \ldots, (s_T, a_T, p_T) \}$.\footnote{While reward-to-go (or other trajectory statistics) are not necessary, we formulate the most general form to showcase how one can easily condition on additional available properties of a trajectory. Using reward-to-go also enables us to compare our method with previous offline-RL work~\citep{chen_decision_2021}.}

Any property of the decision problem can be considered a ``property token'', including specific environment conditions being satisfied, the style of the agent, or the performance of the agent (e.g. the reward obtained in the timestep). Motivated by canonical problems in decision making that involve reward, in almost all of our analysis we consider the return-to-go (RTG) property (the sum of rewards from timestep $t$ to the end of the episode): that is, we set $p_t=\hat{R}_t$ where $\hat{R}_t = \sum_{t' = t}^T r_{t'}$.

\subsection{Tasks as Masking Schemes}\label{sec:masking_schemes}
\orrp{rename title if we do use subsubsections (space constraints will decide)}

In the \fb{} framework, we formulate tasks in sequential decision problems as input masking schemes. Formally, a masking scheme specifies which input tokens are masked (determining what tokens are shown to the model for prediction) and which outputs of the model are masked before computing losses (determining which outputs the model should learn to predict).
% Formally, with the expression \textit{masking scheme} we refer to a function which randomly assigns \texttt{[MASK]}s to each token in trajectory snippets $\tau_{t:t+k}$ of length $k$ drawn uniformly at random from a dataset of trajectories. Each masking scheme defines both which input tokens are masked (determining what tokens are shown to the model for prediction) and which outputs of the model are masked before computing losses (determining which outputs the model should learn to predict).
%where the model must reconstruct states, actions, and/or rewards conditioned on some observations. 
For example, the masking scheme for BC unmasks (conditions on) $s_{0:t}$ and $a_{0:t-1}$, and the model must predict $a_t$.

In \Cref{fig:tasks}, we illustrate how to unify commonly-studied tasks such as BC, goal and waypoint conditioned imitation, offline RL (reward-conditioned imitation), and dynamics modeling under our proposed representation of tasks as masking schemes. We describe the masking scheme for each of these tasks in detail in \Cref{appx:training_regimes_deets}.

\begin{figure*}[t]
  \vspace{-2.5em}
  \centering
  \includegraphics[width=\textwidth]{images/tasks.jpg}
  \vskip -0.15in
  \caption{\textbf{\fb framework: Representing arbitrary tasks as masking schemes.} For each task, we show the inputs to the model (solid colors) and the outputs the model must predict (translucent colors). For example, in future inference, the model must predict all future states and actions conditioned on the initial states and actions. Here we only display one input masking scheme for each task, even though there might be multiple that are valid or necessary (e.g. BC will have up to T different masking schemes, one for each possible history length---although in practice one would generally use the model with a sliding window).
  }\vspace{-1.5em}
  \label{fig:tasks}
\end{figure*}

\subsection{Model Architecture \& Training Regimes}\label{sec:training}
\begin{figure}[t]
% \vskip -0.2in
\vspace{-1.5em}
\begin{center}
\includegraphics[width=0.4\textwidth]{images/fBiT.jpg}
\vspace{-1.5em}
\caption{The \fb{} model takes in a snippet of a trajectory which is masked according to a masking scheme before inference time. For each input possible masking, there are (many) corresponding tasks of predicting the missing inputs. Above we show an input masking corresponding to conditioning on both reward \textit{and} final (goal) state; we highlight the output corresponding to predicting the agent's next action, i.e. performing the inference $\Prob{a_2 | s_{0:2, T}, a_{0:1}, \hat{R}_0}$.}
\label{fig:fb-model}
\end{center}
\vskip -1.8em
\end{figure}

For our main experiments, we instantiate our \fb framework using the BERT architecture \citep{devlin2018bert} adapted to the sequential decision problem domain, consisting of a positional encoding layer and stacked bidirectional transformer encoder (self-attention) layers (see \Cref{fig:fb-model}). One key difference is that we stack the state, action, and property (e.g. RTG) tokens for each timestep into a single vector. While prior work in sequential decision making had used timestep encoding \citep{chen_decision_2021} (which can be thought of as concatenating each observation with its environment timestep), we found traditional positional encoding \citep{vaswani2017attention, devlin2018bert} to reduce overfitting. For reward-conditioned tasks, in each context window we only feed the first RTG token into the model along with the number of timesteps remaining in the horizon. This information is sufficient for reward-conditioning at inference time, and we found that it outperformed the standard approach of feeding in the RTG token at every timestep \citep{chen_decision_2021,janner_reinforcement_2021}. See \Cref{appx:model_details} for more model details, and \Cref{sec:additional-minigrid-exps} for experiments with an alternative instantiation of \fb with a feedforward neural network architecture.

\subsubsection{Training regimes} \label{subsubsec:tr}

We experiment with four \textbf{training regimes}, illustrated in \Cref{fig:training_regimes} and described below. In each regime, a random trajectory sampled (context) and is masked according to a masking scheme; regimes differ by the masking scheme that is applied.


\newcommand{\goalspacestart}{\vspace{0.06in} \\}
\newcommand{\goalspaceend}{\vspace{0.1in}}
% \newcommand{\goal}[1]{\goalspacestart #1 \goalspaceend}
% \newcommand{\goal}[1]{\begin{itemize} \item #1 \end{itemize}}
% \newcommand{\goal}[1]{\begin{framed} \item #1 \end{framed}}
\newcommand{\goal}[1]{\begin{description} \item[\textnormal{\textit{Intuition:}} ] \textit{#1} \end{description}}

\begin{description}[leftmargin=0.2in]
    \ilabel{tr:single}{\texttt{single-task}} Training on just one of the masking scheme described in \Cref{sec:masking_schemes}.
    \goal{The \fb framework provides a unified interface for all tasks (data pipeline, neural architecture, etc.), where only the masking schemes needs to be varied for different tasks. Using s single masking scheme doesn't use the full power of the framework, so we think of \iref{tr:single} as a baseline training regime.}
    
    \ilabel{tr:multi}{\texttt{multi-task}} Training a single model on multiple masking schemes: each trajectory snippet is masked according to one of the schemes from \Cref{sec:masking_schemes} (chosen at random).
    \goal{A single model should perform well on any of the multiple tasks on which it was trained. Additionally, it might outperform \iref{tr:single} on individual tasks, as the model could learn richer representations of the environment from the additional masking schemes.}
    
    \ilabel{tr:random}{\texttt{random-mask}} Training a single model on a fully randomized masking scheme. For each trajectory snippet, first, a masking probability $\pmask \in [0,1]$ is sampled uniformly at random; then each state and action token is masked with probability $\pmask$; lastly, the first RTG token is masked with probability $1/2$ and subsequent RTG tokens are always masked (see \Cref{sec:rnd-masking} for details).
    \goal{A single model should perform well on \emph{any} sequence inference task, without requiring to specify the tasks of interest at training time. The model may learn richer representations than those of \iref{tr:multi} as it must reason about \emph{all} components of the environment.}
    
    \ilabel{tr:finetune}{\texttt{finetune}} Fine-tune a model pre-trained in \iref{tr:random} on a specific masking scheme.
    \goal{A fine-tuned model benefits from the improved representations obtained from \iref{tr:random}, while specializing to the single task at hand.}
\end{description}

% \begin{training}[\textbf{Single-task.}]\label{tr:single}
% Training on only one of the single-task masking schemes from \Cref{sec:masking_schemes}.
% \end{training}

% The only advantage of \Cref{tr:single} is in offering a single, unified interface for all tasks (data pipeline, neural architecture, etc.), where only the masking schemes needs to be varied for different tasks. Indeed, this is more of a convenience than the focus of this work, and so we view this as a baseline training regime. \orrp{Can be made less wordy.}

% \begin{training}[\textbf{Multi-task}]\label{tr:multi}
% Training a single model with multiple masking schemes. Specifically, in each iteration, sample a uniformly random trajectory snippet and apply one of the masking schemes from \Cref{sec:masking_schemes} (chosen at random).
% \end{training}
% \Cref{tr:multi} aims to train a single model that performs well on any of the multiple tasks on which it was train. Additionally, we expect it might outperform \Cref{tr:single} on single tasks, as the model may learn structure in the data from the additional masking schemes.

% \begin{training}[\textbf{Random \maskings{}}]\label{tr:random}
% Training a single model on a randomized masking scheme. Specifically, in each iteration, sample a uniformly random trajectory snippet and mask each token at random. \orrp{See appendix for more info.}
% \end{training}
% \Cref{tr:multi} aims to train a single model that performs well on \emph{any} sequence inference task, without specifying tasks of interest at training time. We expect the model to learn represenetations even richer than that of \Cref{tr:multi} as the model must reason about \emph{all} components of the environment. However, unlike the previous training regimes, in \Cref{tr:multi} the space of possible \maskings grows exponentially with the trajectory snippet (i.e., context) length; it might grow too large for the model to learn anything at all.

% \begin{training}[\textbf{Finetuning} a random \maskings-pretrained model]\label{tr:finetune}
% Fine-tune a model pre-trained in \Cref{tr:random} on a a specific, single-task masking scheme.
% \end{training}
% \Cref{tr:finetune} takes advantage of the improved representations obtained from \Cref{tr:random} while specializing the model parameters to the single task at hand (without sharing model capacity with other tasks). Performance-wise, this should lead to the best of both worlds of randomized and single-task models. Naturally, a fine-tuned model loses the test-time flexibility enabled by \Cref{tr:multi,tr:random}

% \adnote{cool, we have this framework, what do we do it? (consier calling flexibit a framework, and different models emerge out of different ways of training it); we can train models in various ways, each with potential advantages of convential architectures:

% 2. train on random maskings (only, or in addition to prespecified tasks); % 3. do 1 or 2, but fine-tune on the test task; advantage:..;

\begin{figure}[t]
\vspace{-3.5em}
\begin{center}
\includegraphics[width=0.9\textwidth]{images/training_regimes.png}
\vskip -0.85in
\caption{\textbf{The four training regimes considered in this work:} \protect\iref{tr:single}, \protect\iref{tr:multi}, \protect\iref{tr:random} and \protect\iref{tr:finetune}.}
\label{fig:training_regimes}
\end{center}
\vspace{-1.5em}
\end{figure}

\subsubsection{Hypotheses}

Based on the intuition of the strengths of each training regime, we formulate the following hypotheses:

\begin{description}[leftmargin=*]
    \ilabel{H1}{\textbf{H1}} First training on multiple inference tasks will lead to better performance on individual tasks than only training on that inference task: $\left\lbrace \text{\iref{tr:multi}, \iref{tr:random}, \iref{tr:finetune}} \right\rbrace > \text{\iref{tr:single}}$.
    % \\ Reasoning:
    \ilabel{H2}{\textbf{H2}} Random masks training outperforms training on a specific set of tasks: $\text{\iref{tr:random}} > \text{\iref{tr:multi}}$.
    % \\ Reasoning: the model learns richer representations as it must reason about multiple / all components of the environment.
    %\ilabel{H3}{\textbf{H3}} \iref{tr:random} outperforms \iref{tr:multi} for small context length.\footnote{Unlike \iref{tr:multi}, in \iref{tr:random} the space of possible \maskings grows exponentially with the trajectory snippet (i.e., context) length; it might grow too large for the model to learn anything at all.}
    % \\ Reasoning: representations are richer in a model that reasons about \emph{any} task of the environment (vs. just a handful of tasks); however, the number of potential masks grows exponentially with the context length, so in a large contexts the model will almost surely not see any specific task at hand.
    % \ilabel{H4}{\textbf{H4}} \iref{tr:finetune} outperforms \iref{tr:multi} and \iref{tr:random}.
    % \\ Reasoning: A model trained in \iref{tr:finetune} enjoys richer representations without having multiple tasks share its capacity.
\end{description}

\iref{H1} tests whether models learn richer representations by training on multiple inference tasks. \iref{H2} tests a stronger claim: whether training on \emph{all} possible tasks by randomly sampling masking at training time is better than selecting a set of specific maskings.


%Note that \iref{H1} and \iref{H2} together imply that the performance of a pretrained model improves once it is finetuned to a given task; indeed, this statement is supported by existing literature \cite{todo}.

%As observed in \Cref{subsubsec:tr}, we expect a performance increase in \iref{H1} and \iref{H2} due to the richer representations learned by a model trained on multiple (or all possible) tasks. \iref{H3} is based on the observation that the number of possible tasks covered by \iref{tr:random} grows exponentially with the length of the context; this should benefit a \iref{tr:random}-model in smaller context lengths (again, richer representations), but hinder it  when the space of possible tasks becomes prohibitively large.



% \begin{description}[leftmargin=*]
%     \ilabel{H1}{\textbf{H1}} \iref{tr:finetune}, which the framework to its fullest, outperforms \iref{tr:single}.
%     % \\ Reasoning:
%     \ilabel{H2}{\textbf{H2}} Even \iref{tr:multi} and \iref{tr:random} outperform \iref{tr:single}. 
%     % \\ Reasoning: the model learns richer representations as it must reason about multiple / all components of the environment.
%     \ilabel{H3}{\textbf{H3}} \iref{tr:random} outperforms \iref{tr:multi} for small context length.\footnote{Unlike \iref{tr:multi}, in \iref{tr:random} the space of possible \maskings grows exponentially with the trajectory snippet (i.e., context) length; it might grow too large for the model to learn anything at all.}
%     % \\ Reasoning: representations are richer in a model that reasons about \emph{any} task of the environment (vs. just a handful of tasks); however, the number of potential masks grows exponentially with the context length, so in a large contexts the model will almost surely not see any specific task at hand.
%     % \ilabel{H4}{\textbf{H4}} \iref{tr:finetune} outperforms \iref{tr:multi} and \iref{tr:random}.
%     % \\ Reasoning: A model trained in \iref{tr:finetune} enjoys richer representations without having multiple tasks share its capacity.
% \end{description}
% As observed in \Cref{subsubsec:tr}, we expect a performance increase in \iref{H1} and \iref{H2} due to the richer representations learned by a model trained on multiple (or all possible) tasks. \iref{H3} is based on the observation that the number of possible tasks covered by \iref{tr:random} grows exponentially with the length of the context; this should benefit a \iref{tr:random}-model in smaller context lengths (again, richer representations), but hinder it  when the space of possible tasks becomes prohibitively large.

\orrp{TODO if time permits: a paragraph summarizing the empirical findings would be GREAT!}


% In particular, one could train a single-task \fb{} model only on the maskings that correspond to one task from \Figref{fig:tasks} (that is, training with just one of the masking schemes above -- with the exception of random masking). Alternatively, one could train a single model on all the tasks from \Figref{fig:tasks}, randomly selecting among the single-task masking types above for each sequence in a batch. In an even more extreme approach, one could try to train on even more tasks than those above -- for example with random masking training (which trains on all tasks expressible as inferences within sequence snippets). After such random-masking training, one could further fine-tune the model on specific tasks of interest.

% Which training regime would perform better if, say, we are interested in obtaining the highest performance in a single task? What about if we want a single model to be able to perform $n$ tasks: should we train only with maskings corresponding to those $n$ tasks, or with more maskings? Does training on more tasks reduce or increase the performance on each single task, and if so, by how much? Is it actually possible to train on random maskings and obtain reasonable outputs from the model, however it is queried?

% While this will certainly be context dependent, we hypothesize that: 1) at least in certain cases training with multi-task training will improve performance on a single task of interest relative to a single-task model that was only trained on that task (thanks to improved representations); 2) in all cases, when fine-tuning a multi-task model to the single task of interest, it should be possible to get better performance to a single-task model that was only trained on that task; 3) it will be possible to obtain a single model that can perform any inference on the inputted sequence, in a simple enough setting.



% In \Cref{sec:complex-envs}, we present preliminary experimental results from more complex robotics environments, showcasing that performing random-masking training and fine-tuning can obtain comparable or better reward performance in the behavior cloning task.

==> sections/40-gridworld.tex <==
\section{A Unified Model for Any Inference Task}
\label{sec:gridworld}

We first demonstrate how \iref{tr:random} enables a single \fb{} model to perform arbitrary inference tasks at test-time on a gridworld environment, without the need for task-specific output heads or training schemes that are customized for the downstream task. We then show that \iref{tr:random} does not compromise performance on most specific tasks of interest. Models trained with \iref{tr:random} achieve comparable or better performance to \iref{tr:single} and \iref{tr:multi}-models, and in fact consistently outperform after additional fine-tuning on the task of interest (\iref{tr:finetune}).

\prg {Environment Setup.} We design a fully observable $4\times 4$ gridworld in which the agent should move to a fixed goal location behind a locked door with the MiniGrid environment framework \citep{chevalier2018minigrid}. The agent and key positions are randomized in each episode. The agent receives a reward of $1$ for each timestep it moves closer to the goal, $-1$ if it moves away from the goal, and $0$ otherwise. We train \fb{} models on training trajectories of sequence length $T=10$ from a noisy-rational agent \citep{ziebart_maximum_nodate}.
More detailed information about the environment is in \Cref{sec:doorkey-details}.

\subsection{One Model to Rule Them All}

\begin{figure*}
    \vskip -1em
    \centering
    \includegraphics[width=\textwidth]{images/gridworld.jpg}
    \vskip -1.5em
    \caption{\textbf{A \fb model trained with random masking queried on various inference tasks.} \textbf{(1) Behavioral cloning:} generating an expert-like trajectory given an initial state. \textbf{(2) Goal-conditioned:} reaching an alternative goal.
    %, then the original goal (4,4) and finally navigate to state (4,2) for the last timestep. 
    \textbf{(3) Reward-conditioned:} generating a trajectory that achieves a particular reward. \textbf{(4) Waypoint-conditioned:} reaching specified waypoints (or subgoals) at particular timesteps, e.g. going down on the first timestep instead of immediately picking up the key. \textbf{(5) Backwards inference:} generating a likely \emph{history} conditioned in a final state (by sampling actions and states backwards). Trajectories are shown with jitter for visual clarity.}
    \label{fig:gridworld-results}
    \vskip -1em
\end{figure*}

As shown in \Cref{fig:gridworld-results}, a single \fb{} model trained with \iref{tr:random} can be used for arbitrary inference tasks by conditioning on specific sets of tokens.
Unless otherwise indicated, we take the highest probability action from the model $a_t = \arg\max_{a_t'} \Prob{a_t' \mid s_0, a_0, \ldots, s_t}$, and then query the environment dynamics for the next state $s_{t+1}$.
%In some tasks, trajectories rolled out from the model may not always be consistent with the observed factors (e.g. the model's highest probability trajectory may not reach the conditioned waypoints). In these cases, one could use a search procedure such as beam search to expand several trajectory hypotheses, eliminating the ones that are inconsistent with observed factors, although we did not find this to be necessary in the gridworld examples. We use a simpler procedure explained in \cref{sec:doorkey-details}.
The model can be used for imitation, reward- and goal-conditioning, or as a forward or inverse dynamics model (when querying for state predictions, as in the backwards inference task). If trajectories are labeled with properties at training time, the model can also be used for property-conditioning. In \Cref{fig:property-conditioning}, we show how the model can also be conditioned on \textit{global} properties of the trajectory, such as whether the trajectory passes through a certain position at any timestep.

Qualitatively, these results suggest that the model generalizes across masking schemes, since seeing the exact masking corresponding to a particular task at training time is exceedingly rare (out of $2^T \times 2^T \times 2$ possible state, action, and RTG maskings for a sequence of length $T$).

\subsection{Future State Predictions}
\input{sections/41-gridworld-distribution}

Uses of the \iref{tr:random}-trained \fb{} model are not limited to rolling out new trajectories (requesting inferences about the agent's next action). One can also request inferences for states and actions further into the future: e.g., ``where will the agent be \textit{in 3 timesteps}?''. Given a fixed initial set of observed states, we visualize the distribution of predicted states at each timestep in \Cref{fig:state-viz}. Since we do not roll out actions, querying the model for the predicted state distribution at a particular timestep marginalizes over missing actions; for example, $\Prob{s_1 \mid s_0, s_3, s_6}$ models the possibility that the agent chooses either up or left as the first action. Qualitatively, the state predictions suggest that the model accurately captures the environment dynamics and usual agent behavior; e.g. it correctly models that the agent has equal probability of going up and right at $t=3$ (leading it to the distribution over states at $t=4$), and that the agent must be at position (2, 1) at $t=5$ to reach the door at $t=6$.

%\subsection{How do different training regimes compare?}
\subsection{Measuring Single-Task Performance}

Next, we investigate how a \iref{tr:random} model perform on individual tasks, in comparison to \iref{tr:single} models trained exclusively on the evaluated task.
%If we care about a single task (e.g. goal-conditioned imitation), should we train a model simply on that task? Or can there be advantages to training a general model first, and then fine-tuning it to the task of interest? 
\MicahComment{TODO}For this set of experiments, we primarily consider validation loss as our measure of performance. Validation loss provides a general way to evaluate how well models fit the distribution of trajectories and transitions, which is what we are concerned with for most inference tasks: i.e., ``how well can the network predict the true state or action in the data?'' %, and then also look at rewards for a subset of the tasks.

In \Cref{fig:gridworld-valid-ranks500}, we report validation loss if the model is trained on one task (or multiple tasks) and evaluated on another task. As expected, models trained on one masking (e.g. BC; predicting the next action conditioned on the past) perform poorly when queried with another task (e.g. predicting the previous states conditioned on the final state; past inference).
%\prg{Single-task models do well on their task and poorly on others.} As a simple sanity check, notice that all entries on the diagonal (the single-task models, trained and evaluated on a single task) are among the best at the task (that is, their rescaled loss values are quite low relative to other entries in their column). Given that they use the \fb model architecture, they can be evaluated on tasks that they weren't trained on by changing the input maskings: generally, these single tasks model suffer quite a bit of degradation in performance when evaluated on previously-unseen evaluation tasks. %One exception is behavior cloning and offline-RL (behavior cloning), which seem to only lose a couple percentage points: this is likely an indication that in this environment, the reward information is not very informative

Firstly, we find that \iref{tr:random} training (but not \iref{tr:multi} training) outperforms \iref{tr:single} training on half of the tasks considered, showing that even if one is interested in a single inference task training on many more tasks can sometimes improve performance. Specializing a model trained with \iref{tr:random} via finetuning (\iref{tr:finetune}) leads to the best performance, outperforming \iref{tr:single} on all tasks except BC and forward dynamics. This means that even if one is interested in a single inference task, first training on multiple tasks generally improves performance. Overall, these results do not fully support \iref{H1}, given \iref{tr:multi}'s poor performance and \iref{tr:random}'s performance which is not consistently better than \iref{tr:single}.

We also find that \iref{tr:random} training leads to lower loss values on almost all evaluation tasks relative to \iref{tr:multi}, supporting \iref{H2}: training on additional inference tasks beyond the specific ones of interest can augment performance.

% A potential explanation for this result is that, given the same set of training trajectories, multi-task training serves as a form of data augmentation. Single-task models tended to overfit more quickly than the multi-task models. This observation suggests that the benefit of multi-task training might be particularly helpful in low-data regimes.
% \JessyComment{@Micah I saw this bit and added back in, not sure if it still aligns with your intuition?}\MicahComment{Not really that much anymore -- it seems like we found exactly the same results even while varying the amount of data on the minigrid? That definitely made me update away from the data-augmentation theory}

%\prg{Forward and inverse dynamics.} The forward and inverse dynamics evaluations of multi-task models stick out as being particularly poor performance relative to single-task and fine-tuned models. This is because this simple environment has deterministic dynamics, meaning that with sufficient data (as in this case), it's essentially impossible to overfit (``overfitting is fitting''). Training a model for long enough exclusively on forward dynamics gives loss values quite close to zero. This means that any multi-task model which is trading off between that task and others might fail to overfit quite as dramatically (a gap which can be easily made up for during fine-tuning). In this sense, it might be more appropriate to consider the heatmap without these tasks. Still, we wanted to demonstrate how well our model could perform these tasks, if necessary.

\begin{figure}
    \centering
    \includegraphics[width=0.7\columnwidth]{images/heatmaps/500_heatmap_normalized_no_benchmark.png}
    \vskip -0.8em
    \caption{\textbf{Task-specific validation losses (normalized column-wise).} Each row corresponds to the performance of a single model evaluated in various ways, with the exception of the last row---for which each cell is fine-tuned on the respective evaluation task. Loss values are averaged across six seeds and then divided by the smallest value in each column. Thus, for each evaluation task (i.e., column), the best method has value $1$; a value of 1.5 corresponds to a loss that is 50\% higher than the best model in the column. Note that the performance of a multi-task model on the forwards dynamics task is particularly poor since the environment is deterministic: we should expect overfitting (with a single-task model) to perform the best. See \Cref{sec:additional-minigrid-exps} for more details.}% \sm{can we use wrapfig for this figure? or is it banned}\MicahComment{i believe we can use it -- go ahead and do it if you want!}}
    \label{fig:gridworld-valid-ranks500}
    \vskip -0.8em
\end{figure}
% \MicahComment{eventually we could actuad a demo experiment where we try to infer the distribution of the location of the key at t=0 with a past-prediction model}

\MicahComment{TODO: add info about reward/success metrics (appendix)}

% \subsection{How does this single model compare to single-task ones?}

% \prg{High-data regime: similar or better performance after fine-tuning.} If we fine-tune we can do as well or slightly better than single-task models which were trained on the individual task. Any improvement is simply due to having better representations, gained from training on the extra tasks.

% \prg{Low-data regime: better performance out-of-the-box.} This is thanks to the data augmentation effect. We see that the gap becomes larger.



% \MicahComment{We could add a experiment for this?} We prevent a specific type of masking from ever appearing at training time, and the model still does well.



% \subsection{When can we expect better prediction than alternative models?}

% The main avenues through which one would expect \fb{} to perform better than alternatives is through 1) better representations obtained by multi-task training, and 2) less overfitting, as enabled by the data augmentation effect of multi-task training.

% In our experiments, it seems like 2) is playing a bigger role than 1) [provide evidence]



==> sections/41-gridworld-distribution.tex <==
% \begin{figure*}[t]
% \noindent
% \begin{minipage}[!t]{0.35\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/sa_viz.pdf}
%     \vskip -1.3em
%     \caption{Distribution of states and actions for trajectories in the validation set, vs. trajectories sampled from the model, conditioned on the initial agent position (1,4) and key position (2,2).}
%     \label{fig:sa-viz}
% \end{minipage}%
\begin{figure*}[t]
\noindent
\begin{minipage}[!t]{0.49\textwidth}
    \centering
    \includegraphics[width=0.8\textwidth]{images/property-conditioned.pdf}
    \caption{\textbf{Other types of property-conditioning.} If the training dataset has additional property labels (e.g., whether the trajectory passes by the top left corner of the grid \textit{at any timestep}), the model can roll out trajectories conditioned on whether the property is exhibited.}
    \label{fig:property-conditioning}
    \vskip -2em
\end{minipage}%
\hfill%
\begin{minipage}[!t]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/state_viz.pdf}
    \caption{\textbf{Predicted state distributions.} The model is conditioned on states at $t=0, 3, 6$.}
    \label{fig:state-viz}
    \vskip -2em
\end{minipage}%
\end{figure*}

==> sections/50-complex-tasks.tex <==
\section{Trajectory Generation in a Complex Environment}\label{sec:complex-envs}

In addition to gridworld, we test our method in a partially observable, continuous-state and continuous-action environment, with a larger trajectory horizon (200 timesteps).\JessyComment{add some more intro here that links to the new title}

\subsection{Environment Setup}
We adapt the Mujoco-physics Maze2D environment~\cite{fu2020d4rl} (see \Cref{sec:maze-details} for figures), in which a point-mass object is placed at a random location in a maze, and the agent is rewarded for moving towards a randomly generated target location (making this task ``goal-conditioned by default'').
% The timestep-reward is the percentage of distance covered between the initial position and the target position -- this has the advantage of leading to interpretable cumulative rewards: $70$ means that the agent was able to get $70\%$ of the way towards the goal. 
We make this task harder by removing the agent's velocity information from each timestep's observation and increasing the amount of initial position randomization. These changes make the environment partially observable, forcing models trained on this data to implicitly infer the agent's velocity from observed context.

\prg{Expert dataset.} We want our expert data to have some suboptimality so that reward-conditioning can be tested for better-than-demonstrator performance.
We generate a dataset of expert trajectories by rolling out D4RL's PD controller (which is non-Markovian), and add noise to the actions with zero-mean and $0.5$ variance (which are then clipped to have each dimension between $-1, 1$). We generate 1000 trajectories of 200 timesteps, of which 900 are used for testing and 100 for validation. For more details on our adapted Maze2D environment and design decisions, see \Cref{sec:maze-details}.

\subsection{Models Trained}

For the Maze2D evaluations, we focus on test-time reward performance on behavior cloning and offline RL (reward-conditioning) across various architectures and training regimes.

We consider \fb models trained with the different training regimes: \iref{tr:single}, \iref{tr:multi}, \iref{tr:random}, and \iref{tr:finetune}. We additionally consider other architectures, such as a feed-forward NN and Decision Transformer (DT) baselines \citep{chen_decision_2021}.
We found that several of our design decisions for \fb models -- using positional encoding instead of timestep encoding, inputting the return-to-go token at the first timestep with the number of timesteps in the horizon -- also improved GPT-based models like DT.
%also developed a stronger baseline than DT which was obtained by transferring many design choices that benefited \fb to a GPT-based model.
We call our improved baseline Decision-GPT (for implementation details, see \Cref{sec:gpt-details}). We train our Decision-GPT model with the \iref{tr:single} training regime.
The only meaningful difference between Decision-GPT and a \iref{tr:single} \fb model is whether the model is GPT- or BERT-based.

For each architecture and applicable training regime, we train separate models to perform behavior cloning and offline RL (reward-conditioning). The only exceptions are \fb models trained with \iref{tr:multi} (trained to perform BC and RC) and \iref{tr:random}. We train two sets of such models, for context lengths of 5 and 10 -- meaning that during both training and evaluation, the models will respectively only be able to see the last 5 or 10 timsteps of the agent's interaction with the environment.

\subsection{Results}

We report reward evaluation results for 1000 rollouts in the Maze environment with standard errors across 5 seeds in \Cref{table:maze_results}.

\prg{The value of pre-training and fine-tuning for \fb models.} We find that fine-tuning is critical for good performance in more complex environments. 
\iref{tr:multi} performs comparably to \iref{tr:single} in behavior cloning and reward conditioning; however, \iref{tr:random} in this setting suffers in terms of reward-performance (counter to \iref{H2}). This suggests that \iref{tr:multi} training can be effective in increasing reward performance, but training on too many tasks can hurt out-of-the-box performance. However, \iref{tr:finetune} recovers the performance loss, again out-performing \iref{tr:single} (providing qualified support for \iref{H1}). Surprisingly, fine-tuning \iref{tr:multi} does not improve performance as much as fine-tuning the randomly masked model, suggesting that specifically training on random masking provides benefits for adapting models to individual downstream tasks.

%Across \fb models, \iref{tr:finetune} consistently leads to the highest reward (supporting \iref{H1}). We see that \iref{tr:multi} on performs comparably to \iref{tr:single} in behavior cloning and reward conditioning; however, \iref{tr:random} in this setting suffers in terms of reward-performance. This suggests that \iref{tr:multi} training can be effective in increasing reward performance, but training on too many tasks can hurt---supporting \iref{H2}. 


% However, our results go against \iref{H3}, since we used a fairly short context lengths of give. This might be due to capacity constraints of the networks; it may not being able to learn how to perform all tasks at once without trading off on performance. It may also be an optimization issue \orrp{Say more re optim, or don't say it at all.}

\prg{How do \fb models compare to other architectures?} For context length five, we see that \iref{tr:finetune} \fb models perform better than all baselines we consider. However, increasing the context length to ten, we see that \fb models performs poorly across the board, with \iref{tr:finetune} outperformed even by our Decision-GPT baseline. We speculate that this might be related to the documented difficulty of using BERT-like architectures (as that of \fb models) for sequence generation \citep{wang2019bert, mansimov2019generalized}.% without additional tricks \citep{Ghazvininejad2019MaskPredictPD} to increase output likelihood -- which are not applicable in our domain (because we want to match the data distribution instead of having maximum likelihood trajectories).\MicahComment{add more cites}

\prg{Isolating the effect of GPT vs. BERT.} In order to investigate the effect of using GPT-like architectures instead of BERT-like ones, we can consider the comparison between \iref{tr:single} \fb and our Decision-GPT baseline: the main difference between these two models is only whether one uses BERT or GPT as the backbone of the architecture.\footnote{We additionally use input-stacking for \fb---see \Cref{appx:model_details}---but in preliminary experiments we found this to not affect performance.} We find that while using GPT seems to yield similar performance to BERT for context length five, using GPT seems to give an advantage for longer sequence lengths. In particular, note that a larger context length enables GPT to increase performance, while this is not the case for \iref{tr:single} \fb. This suggests that if one were able to use a GPT architecture and train it with random masking and fine-tuning, it might be possible to get the best of both worlds.

\begin{table}[h]
\centering
\vskip -2em
\caption{\textbf{Maze2D Results.} \textbf{Comparing among \fb models}, we isolate the benefit of \protect\iref{tr:random}: this training regime performs best across tasks and sequence lengths. \textbf{Comparing \protect\iref{tr:single} \fb to our Decision-GPT model}, we can isolate the effect of using a BERT-like architecture vs. a GPT-like architecture: for larger context lengths, BERT-like models struggle to maintain the same generation quality, while our Decision-GPT model effectively makes use of the extra context. Every entry in the table corresponds to separate training runs (trained on either BC or RC), except for the cells denoted with $^\dagger$, which are shared across tasks (but not sequence lengths).}\label{table:maze_results}
\begin{tabular}{@{}l|ll|ll@{}}

\MicahComment{Have fancy table arrows}

              & \ \ Ctx. len 5 &  & \ \ Ctx. len 10 &  \\ \toprule
\textbf{Model} & BC & RC & BC & RC \\ \midrule
% Data & $1.82  $ & $n/a$ \\ \midrule
\textbf{\fb Models} \\
\fb- \iref{tr:single} & $2.71\pm .02  $ & $2.63 \pm .02$ & $2.50 \pm .03$ & $2.42 \pm .04$ \\
\fb- \iref{tr:multi} (BC \& RC) & $2.71 \pm .01^\dagger$ & $2.71 \pm .02^\dagger$ & $2.48 \pm .03^\dagger$ & $2.47 \pm .04^\dagger$\\
\fb- \iref{tr:multi} + finetune & $2.72 \pm .05$ & $2.72 \pm .02$ & $2.45 \pm .05$ & $2.46 \pm .06$\\
\fb- \iref{tr:random} & $2.11 \pm .06^\dagger$ & $2.14 \pm .09^\dagger$ & $2.29 \pm .08^\dagger$ & $2.30 \pm .08^\dagger$\\
% \fb-RND$_{BC}$ & $2.49  $ & $n/a$  & $2.28  $ & $n/a$\\ \midrule
\fb- \iref{tr:finetune} & $\mathbf{2.74 \pm .06} $ & $\mathbf{2.73\pm .04} $ & $\mathbf{2.67 \pm .04}$ & $\mathbf{2.64 \pm .05}$\\\midrule
% \fb-RND$_{BC}$ - Finetune & $\mathbf{2.76} $ & $\mathbf{2.75} $ & $2.64 $& $2.63 $\\ 
\textbf{Other architectures} \\
Feedforward Neural Network & $1.62 \pm .05$ & $1.60 \pm .05$ & $1.82 \pm .07 $ & $1.83 \pm .05$\\
Decision Transformer \citep{chen_decision_2021} & $1.33 \pm .03$ & $1.50\pm .04$ & $1.99 \pm .02$ & $1.76 \pm .04$ \\
Our Decision-GPT model & $2.61\pm .01 $ & $2.35\pm .03$ & $\mathbf{2.75\pm .02}$ & $\mathbf{2.74 \pm .02}$\\ 
\bottomrule
\end{tabular}
\vskip -0.5 em
\end{table}


% \MicahComment{using neural network rather than transformer with maskings}
% \MicahComment{ablation on stacking}
% \MicahComment{ablation on first-reward}

% \MicahComment{try larger seq len}
% \MicahComment{try larger maze env}
% \MicahComment{try more data}
% \MicahComment{do more hyperparam tuning}
% \MicahComment{re-run medium with split which has worse average performance?}
% \MicahComment{try fine-tuning}

==> sections/60-limitations-conclusion.tex <==
\section{Limitations and Future Work} \label{sec:lim_and_future}
% \prg{Offline RL.} Although offline-RL is used in this paper just as a means to display our model's flexibility, confronting the issues in the Mujoco environments described in \secref{} made us confront various questions: what do we intend our learners to do when they are presented with a very small amount of data (e.g. a single trajectory) to learn from? If environments are amenable to achieving high reward through memorization/regurgitation of expert trajectories - should we steer away from this path or embrace it? Do we have expectations that an offline RL method will be able to generalize beyond the set of states it has seen in the training data? \MicahComment{it's not just about this -- also in general: are low randomness environments good indicators of performance? are any of the comparisons we gain in that domain meaningful, or just capture a model's capability of memorizing/regurgitating data?}

% Hyperparameter Selection for Imitation Learning - imitation learning MSE / reward.

\prg{Comparison to other specialized models.}
We show that \fb{} outperforms feedforward networks, Decision Transformer models, and for short sequence lengths also our own improved GPT-based baseline. However, we do not compare our models directly to different models in prior work that are specialized for specific tasks (e.g. goal-conditioning models, etc.). While this is a limitation of our work, it is also not our main focus: we propose a unifying framework for a variety of tasks in sequential decision problems, and extensively analyze how different training regimes affect performance. %We test our method in both a simple discrete minigrid environment and a more challenging continuous-control, partial-information \MicahComment{we don't actually call it partial info before, but i think it is?} Maze navigation environment. While these environments  \MicahComment{update}

% \prg{Property-conditioning.} The choice of representing trajectories as states, actions, and returns-to-go is not constrained by the model. One could use any property of the environment or the agent as additional tokens (or set of tokens), enabling to perform property-conditioned inferences, or infer such properties from test-time trajectory snippets. Reward-conditioning is just one example of such property-conditioning \citep{zhan2020learning, furuta2021generalized}. \MicahComment{update}

\prg{Longer context lengths.} One limitation in our experimentation is the relatively short context lengths used. %This is because 1) the architecture we use requires memory quadratic in the sequence length, and 2) the number of possible random maskings is exponential in the sequence length.
% In addition to reducing the expressivity of the model, using short sequence lengths reduces the applicability of maskings such as goal and waypoint conditioning (which can only condition on future states within the context window).
%1) could be addressed by using efficient transformers~\citep{wang2020linformer, jaegle2021perceiver}; 2) 
We found that longer context lengths negatively affect the \fb models' performance. In part, this could be addressed by designing masking schemes tailored to specific test-time tasks (see \Cref{sec:rnd-masking}), or using principled masking schemes \citep{levine2020pmi}. However, this degradation may be attributed to our use of a BERT-like (rather than GPT-like) architecture, which seems less compatible with longer sequence lengths. A clear avenue of future work would therefore be to get the ``best of both worlds'': long sequences and benefits of \iref{tr:random} pre-training by using a GPT-like architectures, with our \iref{tr:random} and \iref{tr:finetune} training regimes. This would require finding ways to make GPT act like a bidirectional model -- for which recent methods in NLP  might offer a useful starting point \citep{aghajanyan2022cm3, fried2022incoder}. \MicahComment{Idea behind Prefix LMs \cite{UL2}}

% A clear future direction is to try to get the best of both worlds, by using both GPT and this idea of randomized training.
% Comparing between DT* and UniBiT is “somewhat unfair” in the sense that we’re also strengthening our baseline (maybe we should call it something different?). Note that if we only compared to DT, we would achieve better results than DT on reward-conditioning also in sequence length 10.\MicahComment{clean up, space to claim that GPT-rnd is another paper.}

\prg{Other future work.} In order to speed up training time efficiency, one could try to substitute BERT for XLNet or NADE-style approaches \citep{yang_xlnet_2020, Uria2016NeuralAD}. Another exciting direction for future work is determining whether the benefits obtained from \iref{tr:random} (or even \iref{tr:multi}) apply to other types of inferences more generally (e.g. Bayes Networks); alternatively, even trivially extending the approach to multi-agent settings (for which token-stacking could prove more valuable), could enable many interesting masking-enabled queries \cite{ngiam_scene_2021}. %More work on understanding what information BERT learns, and how it is stored, and whether and how multi-task training improves representations in the setting of sequential decision problems also seems warranted \citep{Rogers}.

% Additionally, we propose a flexible way of handling inputs that enables us to substantially increase the sequence length that is feasible to handle by our model relative to previous work \citep{chen_decision_2021, janner_reinforcement_2021}.

% Syntetic demonstrations are not necessarily good proxy for human data (sec 5 \citep{orsini2021matters})


\section{Conclusion}\label{sec:conclusion}

\prg{Broader impacts.} The prospect of very large ``foundation models'' \citep{foundation} becoming the norm for sequential problems (in addition to language) raises concerns, in that it de-democratizes development and usage \citep{Kalluri2020}. We use significantly smaller models and computational power than similar works, leaving open the option to have more modestly-sized environment-specific foundation models. However, we acknowledge that this works still encourages this trend.

\prg{Summary.} In this work we propose \fb, a framework for flexibly defining and training models which: \textbf{1)} are naturally able to represent any inference task and support multi-task training in sequential decision problems, \textbf{2)} match or surpass the performance of single-task models after multi-task pre-training, and almost always surpasses them after fine-tuning. We believe our approach provides an elegant conceptual formulation and exciting experimental results which warrant further investigation by the research community.

% \MicahComment{replace all mentions of IL/imitation learning with BC/behavior cloning}

==> sections/69-checklist.tex <==
\section*{Checklist}



% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{} 
  \item Did you describe the limitations of your work?
    \answerYes{See \Cref{sec:lim_and_future}.} 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See \Cref{sec:conclusion}.} 
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code is linked at the top of the Appendix.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See the relevant Appendix sections, for each environment and model.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Yes, with the exception of \Cref{fig:gridworld-valid-ranks500}. More details in \Cref{sec:additional-minigrid-exps}}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{See the relevant Appendix sections.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Yes, our codebase is linked in the appendix as a URL.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

